Folding Attention: Memory and Power Optimization for On-Device Transformer-based Streaming Speech Recognition

Transformer-based models excel in speech recognition. Existing efforts to optimize Transformer inference, typically for long-context applications, center on simplifying attention score calculations. However, streaming speech recognition models usually process a limited number of tokens each time, making attention score calculation less of a bottleneck. Instead, the bottleneck lies in the linear projection layers of multi-head attention and feedforward networks, constituting a substantial portion of the model size and contributing significantly to computation, memory, and power usage. To address this bottleneck, we propose folding attention, a technique targeting these linear layers, significantly reducing model size and improving memory and power efficiency. Experiments on on-device Transformer-based streaming speech recognition models show that folding attention reduces model size (and corresponding memory consumption) by up to 24% and power consumption by up to 23%, all without compromising model accuracy or computation overhead.

==> datasets.tex <==
\subsection{Datasets}
\label{subsec:datasets}

We conducted experiments on two datasets: LibriSpeech~\cite{librispeech} and an in-house dataset.\vspace{2em}

\noindent\textbf{LibriSpeech:} We used 960 hours of its training dataset, extracting 80-dimensional log Mel-filterbank features every 25 milliseconds, with a sliding window of 10 milliseconds. Following the Emformer Transducer work~\cite{emformer}, we used a pre-trained sentence piece model~\cite{kudo2018sentencepiece} to produce 4096-dimensional sentence pieces, plus an additional ``blank'' symbol, as our Transducer models predict. We used \textit{test-clean} and \textit{test-other}, the test sets of Librispeech, for evaluating the model accuracy.\vspace{1em}

\noindent\textbf{In-house dataset:} It consists of 23k hours of data sampled from English public videos. The audio was de-identified and aggregated, with personally identifiable information (PII) removed. We distorted the collected audio using simulated reverberation and added randomly sampled additive background noise extracted from publicly available videos. We applied speed perturbations~\cite{ko15_interspeech} to create two additional copies of the training datasets at 0.9 and 1.1 times the original speed. We further applied distortion and additive noise to the speed-perturbed data. This resulted in a total of 127.8k hours of training data. For evaluating the accuracy of models trained on this dataset, we use the following two test sets:
\begin{itemize}
\item \textit{dictation:} 5.8k hand-transcribed, de-identified, and aggregated utterances from vendor-collected data where speakers were asked to record unscripted open-domain dictation conversations. The audio was recorded in a variety of noise conditions and speaking volumes.
\item \textit{messaging:} 13.4k hand-transcribed, de-identified, and aggregated utterances from vendor-collected data where speakers were asked to record audio messages for an unspecific person based on a scripted scenario. These utterances are generally shorter and have a higher signal-to-noise ratio (SNR) than the dictation dataset.
\end{itemize}



